Fast Training Dataset Attribution via In-Context Learning

We investigate the use of in-context learning and prompt engineering to estimate the contributions of training data in the outputs of instruction-tuned large language models (LLMs). We propose two novel approaches: (1) a similarity-based approach that measures the difference between LLM outputs with and without provided context, and (2) a mixture distribution model approach that frames the problem of identifying contribution scores as a matrix factorization task. Our empirical comparison demonstrates that the mixture model approach is more robust to retrieval noise in in-context learning, providing a more reliable estimation of data contributions.

==> conclu.tex <==
Our results show that both of our proposed algorithms successfully attribute the output of LLMs to the BoolQ dataset (as a proxy for related knowledge). Comparison of LLMs GPT-4 showed minimal change in similarities when the BoolQ context was added, suggesting prior exposure to similar data, while Bloomz exhibited a high residual, indicating substantial influence from BoolQ. The CMF algorithm provides further insight by quantifying the contributions of the base LLM. Comparing our two methods, we conclude that CMF is computationally less expensive and more robust to the RAG noise.

%In this paper, we consider several datasets as proxies for the datasets used for LLM training. For future work, we will try to avoid this approximate method and train our LLMs on specific datasets and test our algorithms with ground truth-contributing datasets obtained by retraining.

%The Shapley-normalized residual similarities approach highlighted the LLMs' performance differences with additional context, providing insights into their training exposures. However, it was computationally intensive and less prone to RAG noise. Conversely, the mixture distribution model offered a more efficient and robust method, with less computational overhead and reduced sensitivity to RAG noise.

% Overall, our findings validate the proposed methodologies for quantifying dataset contributions, offering a framework that enhances understanding of data attribution in model training. Future work could focus on refining these methods and exploring their applicability to a broader range of datasets and LLMs.

